The DIRAC code for relativistic molecular calculations

DIRAC is a freely distributed general-purpose program system for 1-, 2- and 4-component relativistic molecular calculations at the level of Hartree--Fock, Kohn--Sham (including range-separated theory), multiconfigurational self-consistent-field, multireference configuration interaction, coupled cluster and electron propagator theory. At the self-consistent-field level a highly original scheme, based on quaternion algebra, is implemented for the treatment of both spatial and time reversal symmetry. DIRAC features a very general module for the calculation of molecular properties that to a large extent may be defined by the user and further analyzed through a powerful visualization module. It allows the inclusion of environmental effects through three different classes of increasingly sophisticated embedding approaches: the implicit solvation polarizable continuum model, the explicit polarizable embedding, and frozen density embedding models. DIRAC was one of the earliest codes for relativistic molecular calculations and remains a reference in its field.

==> gfx/adcmat_pgf.tex <==
\begin{tikzpicture}[scale=1.3]
    \footnotesize
    %\draw [help lines] (-1,0) grid (23,5);
    \draw [thick] (0,0) rectangle (3,3);
    \draw [thick] (0,2) rectangle (1,3) node [midway] {0,1,2,2,3};
    \draw [thick] (1,0) rectangle (3,2) node [midway] {--,--,0,1,1};
    \draw [thick] (0,0) rectangle (1,2) node [midway] {--,--,1,1,2};
    \draw [thick] (1,2) rectangle (3,3) node [midway] {--,--,1,1,2};
    \node (1h1) at (0.5,3.5) {1h};
    \node (1h2) at (-0.5,2.5) {1h};
    \node (2h1) at (2.0,3.5) {2h1p};
    \node (2h2) at (-0.5,1.0) {2h1p};

\end{tikzpicture}

